Multi-Reference Generative Face Video Compression with Contrastive Learning

Generative face video coding (GFVC) has been demonstrated as a potential approach to low-latency, low bitrate video conferencing. GFVC frameworks achieve an extreme gain in coding efficiency with over 70% bitrate savings when compared to conventional codecs at bitrates below 10kbps. In recent MPEG/JVET standardization efforts, all the information required to reconstruct video sequences using GFVC frameworks are adopted as part of the supplemental enhancement information (SEI) in existing compression pipelines. In light of this development, we aim to address a challenge that has been weakly addressed in prior GFVC frameworks, i.e., reconstruction drift as the distance between the reference and target frames increases. This challenge creates the need to update the reference buffer more frequently by transmitting more Intra-refresh frames, which are the most expensive element of the GFVC bitstream. To overcome this problem, we propose instead multiple reference animation as a robust approach to minimizing reconstruction drift, especially when used in a bi-directional prediction mode. Further, we propose a contrastive learning formulation for multi-reference animation. We observe that using a contrastive learning framework enhances the representation capabilities of the animation generator. The resulting framework, MRDAC (Multi-Reference Deep Animation Codec) can therefore be used to compress longer sequences with fewer reference frames or achieve a significant gain in reconstruction accuracy at comparable bitrates to previous frameworks. Quantitative and qualitative results show significant coding and reconstruction quality gains compared to previous GFVC methods, and more accurate animation quality in presence of large pose and facial expression changes.

==> ref.tex <==

\begin{thebibliography}{00}

%2D Animation
\bibitem{b1} A. Siarohin and S. Lathuili{\`e}re, S. Tulyakov and E. Ricci, and N. Sebe, "First order motion model for image animation", NeurIPS, 2019

\bibitem{b2} E. Zakharov,I. Aleksei , A. Shysheya and V. Lempitsky, "Few-Shot Adversarial Learning of Realistic Neural Talking Head Models", ICCV, 2019 

%3D Face reconstruction
% \bibitem{b5} E. Wood, T. Baltrusaitis, C. Hewitt, M. Johnson, J. Shen, N. Milosavljevic, D. Wilde, S. Garbin, C. Raman, J.Shotton, T.Sharp, I. Stojiljkovic and T. Cashman, J. Valentin, "3D face reconstruction with dense landmarks", ECCV, 2022

% \bibitem{b6} Y. Feng, H. Feng, M. J. Black and T. Bolkart, "Learning an animatable detailed 3D face model from in-the-wild images", ACM Transactions on Graphics, 2020


% \bibitem{b8} L. Guo, H. Zhu, Y. Lu, M. Wu and X. Cao, "RAFaRe: Learning Robust and Accurate Non-parametric 3D Face Reconstruction from Pseudo 2D\&3D Pairs",
% AAAI Conference on Artificial Intelligence,
% 2023

% Animation-based coding
\bibitem{b3} G. Konuko, G. Valenzise, and S. Lathuiliere, "Ultra-low bitrate video conferencing using deep image animation",
IEEE ICASSP, 2020

\bibitem{b4} G. Konuko, G. Valenzise, and S. Lathuiliere, "A Hybrid Animation Codec for low bitrate video conferencing",
IEEE ICIP, 2022

\bibitem{b5} G. Konuko, G. Valenzise, and S. Lathuiliere, "Predictive coding for animation-based video compression",
IEEE ICIP, 2023

\bibitem{b6} T. Wang, A. Mallya, M. Liu, "One-Shot Free-View Neural Talking-Head Synthesis for Video Conferencing", CVPR, 2021

\bibitem{b7} M. Oquab,P. Stock, O. Gafni,D. Haziza, T. Xu, P. Zhango and O. Celebi, "Low Bandwidth Video-Chat Compression using Deep Generative Models", CVPR, 2021

\bibitem{b8} B. Chen, Z. Wang, B. Li, R. Lin,S. Wang and Y. Ye, "Beyond Keypoint Coding: Temporal Evolution Inference with Compact Feature Representation for Talking Face Video Compression", DCC, 2022

\bibitem{b9} Z. Chen and M. Lu, H. Chen and Z. Ma, "Robust Ultra-low Bitrate Video Conferencing with Second Order Motion Coherency", MMSP, 2022

%Conditional residual coder
\bibitem{b10} F. Brand, J. Seiler and A. Kaup, "Conditional Residual Coding:
A Remedy for Bottleneck Problems in
Conditional Inter Frame Coding",arxiv preprint, 2023


%conventional codecs
\bibitem{b11} G. Sullivan, J. Ohm ,W. Jin and T. Wiegand, "Overview of the high efficiency video coding (HEVC) standard", IEEE TCSVT, 2012

\bibitem{b12} B. Bross and J. Chen, J. Ohm and G. Sullivan
and Y. Wang, "Developments in inter-
national video coding standardization after avc, with an
overview of versatile video coding (VVC)", Proceedings of the IEEE, 2021

%learned codecs

\bibitem{b13} G. Lu, W. Ouyang, D. Xu, X. Zhang, C. Cai and Z. Gao, "Dvc: An end-to-end deep video compression framewor", CVPR, 2019

\bibitem{b14} J. Li, B. Li and Y. Lu,
"Deep contextual video compression", NeurIPS, 2021

\bibitem{b15} T. Ladune and P. Philippe, "AIVC: Artificial Intelligence based Video Codec",ICIP, 2022 

%metrics
\bibitem{b16} K. Simonyan and A. Zisserman, "Very deep convolutional networks for large scale image recognition", ICLR, 2015

\bibitem{b17} R. Zhang, P. Isola and A. Efros, E. Shechtman  and O. Wang,"The Unreasonable Effectiveness of Deep Features as a Perceptual Metric",CVPR, 2018

\bibitem{b18} K. Ding, K. Ma, S. Wang and E. Simoncelli, "Image Quality Assessment: Unifying Structure and Texture Similarity", IEEE Transactions on Pattern Analysis and Machine Intelligence, 2022

\bibitem{b19}J. Ball{\'e}, V. Laparra and E. Simoncelli,"End-to-end optimized image compression", NeurIPS, 2016

\bibitem{b20} Interdigital.inc, "https://interdigitalinc.github.io/CompressAI/",2023

\bibitem{b21} Z. Cheng, H. Sun, M. Takeuchi, J. Katto, "Learned Image Compression with Discretized Gaussian Mixture Likelihoods and Attention Modules",
CVPR,2020

\bibitem{b21} A. Volokitin, S. Brugger, A. Benlalah, S. Martin, B. Amberg, M. Tschannen,"Neural Face Video Compression using Multiple Views",
CVPR Workshop, 2022

\bibitem{b22} Z. Wang, B. Chen, Y. Ye,S. Wang,
"Dynamic Multi-Reference Generative Prediction for Face Video Compression",
ICIP, 2022

\bibitem{b23}
H. Le-Khac, G. Healy,F. Smeaton,
"Contrastive Representation Learning: A Framework and Review",
IEEE Access, 2020

\bibitem{b24}
T. Chen,S. Kornblith,M. Norouzi, G. Hinton, "A simple framework for contrastive learning of visual representations",
JMLR.org, 2020,
\end{thebibliography}
